Accelerating Kernel Classifiers Through Borders Mapping

Support vector machines (SVM) and other kernel techniques represent a family of powerful statistical classification methods with high accuracy and broad applicability. Because they use all or a significant portion of the training data, however, they can be slow, especially for large problems. Piecewise linear classifiers are similarly versatile, yet have the additional advantages of simplicity, ease of interpretation and, if the number of component linear classifiers is not too large, speed. Here we show how a simple, piecewise linear classifier can be trained from a kernel-based classifier in order to improve the classification speed. The method works by finding the root of the difference in conditional probabilities between pairs of opposite classes to build up a representation of the decision boundary. When tested on 17 different datasets, it succeeded in improving the classification speed of a SVM for 12 of them by up to two orders-of-magnitude. Of these, two were less accurate than a simple, linear classifier. The method is best suited to problems with continuum features data and smooth probability functions. Because the component linear classifiers are built up individually from an existing classifier, rather than through a simultaneous optimization procedure, the classifier is also fast to train.

==> svm_accel_rev1_symbol_table.tex <==
%list of symbols as a latex table

\begin{tabular}{lll}
symbol & definition & first used \\ \hline
	$\lindecision$ & decision function in linear classifier & (\ref{linear_classifier})\\
	$\bordernormal$ & hyperplane normal of decision boundary & (\ref{linear_classifier})\\
	$\borderconst$ & constant value defining location of decision boundary & (\ref{linear_classifier})\\
	$\testpoint$ & test point & (\ref{linear_classifier})\\
	$\sample_i$ & features data for $i$th training sample & \S \ref{theory} \\
	$\classlabel_i$ & class label of $i$th training sample & \S \ref{theory} \\
	$\nsample$ & number of training samples & \S \ref{theory} \\
	$\svmdecision$ & raw decision function in binary SVM & (\ref{svm_decision})\\
	$\vectorkernel$ & kernel function & (\ref{svm_decision})\\
	$\lbrace \svmcoeff_i \rbrace$ & coefficients in SVM & (\ref{svm_decision})\\
	$\class$ & class label & (\ref{class_value})\\
	$\svmcost$ & cost parameter in SVM for reducing over-fitting & (\ref{constraint1}) \\
	$\svmprob$ & LIBSVM estimator for $\diffcondprob$ & (\ref{svm_prob}) \\
	$\svmprobcoeffA$ & coefficient used in $\svmprob$ & (\ref{svm_prob}) \\
	$\svmprobcoeffB$ & coefficient used in $\svmprob$ & (\ref{svm_prob}) \\
	%$\kernelparam$ & parameters in vector kernel & (\ref{kernel_estimator})\\
	%$\point=\lbrace \coord_i \rbrace$ & point in the feature space & (\ref{norm_def})\\
	$\condprob(\class|\point)$ & conditional probability & (\ref{rdef}) \\
	$\diffcondprob$ & difference in conditional probabilities for binary classifier & (\ref{rdef}) \\
	$\decisionfunction$ & decision function which is estimator of $\diffcondprob$ & (\ref{rdef})\\
	$\lbrace \bordervector_i \rbrace$ & set of vectors defining the class border & (\ref{border_decision}) \\
	$\lbrace \bordernormal_i \rbrace$ & set of normals to the class border & (\ref{border_decision}) \\
	$\nborder$ & number of border vectors & (\ref{border_decision}) \\
	$\borderdecision$ & raw decision function for border classification & (\ref{border_decision}) \\
	$\borderprob$ & borders estimator for $\diffcondprob$ & (\ref{border_probability}) \\
	$\multiprob_i=\condprob(i|\point)$ & conditional probability of $i$th class & (\ref{bin2multi}) \\
	$\nclass$ & number of classes & (\ref{bin2multi}) \\
	$\lmult$ & Lagrange multiplier in multi-class problem & (\ref{multiclass}) \\
	$\lbrace \confusion_{ij} \rbrace$ & confusion matrix & (\ref{accuracy}) \\
	$\ntest$ & number of test points & (\ref{accuracy}) \\
	$\priorentropy$ & entropy of the prior distribution & (\ref{prior_entropy}) \\
	$\posteriorentropy$ & entropy of the posterior distribution & (\ref{posterior_entropy}) \\
	$\UC$ & uncertainty coefficient (normalized channel capacity) & (\ref{uncertainty_coefficient}) \\
%symbol & definition & first used \\ \hline
	$\dimension$ & number of dimensions in feature space & (\ref{scaling_law})\\
	$\featurevolume$ & volume of the feature space occupied by training data & (\ref{scaling_law}) \\
	$\mintrain$ & number of training samples needed for good accuracy & (\ref{scaling_law}) \\
	$\minborders$ & number of border samples needed for good accuracy & (\ref{scaling_law}) \\
	$\rbkernelparam$ & parameter for Gaussian (RBF) kernel in SVM & \S \ref{results_section} \\
	$\datafraction$ & fraction of data used for testing & \S \ref{results_section} \\
	$\classsize_i$ & size of $i$th class & (\ref{subsample}) \\
	$\subsample$ & subsampling fraction as function of class size & (\ref{subsample}) \\
	$\subexp$ & exponent in subsampling function $\subsample$ & (\ref{subfunction}) \\
	$\submultcoef$ & coefficient in subsampling function $\subsample$ & (\ref{subfunction}) \\
\end{tabular}


